Managing Latency in Edge-Cloud Environment

Modern Cyber-physical Systems (CPS) include applications like smart traffic, smart agriculture, smart power grid, etc. Commonly, these systems are distributed and composed of end-user applications and microservices that typically run in the cloud. The connection with the physical world, which is inherent to CPS, brings the need to operate and respond in real-time. As the cloud becomes part of the computation loop, the real-time requirements have to be also reflected by the cloud. In this paper, we present an approach that provides soft real-time guarantees on the response time of services running in cloud and edge-cloud (i.e., cloud geographically close to the end-user), where these services are developed in high-level programming languages. In particular, we elaborate a method that allows us to predict the upper bound of the response time of a service when sharing the same computer with other services. Importantly, as our approach focuses on minimizing the impact on the developer of such services, it does not require any special programming model nor limits usage of common libraries, etc.

==> developer_perspective.tex <==
In this section, we outline our approach from the perspective of a developer of edge-cloud microservices. First we focus on submission to the cloud then to what is the probe and in the last part we provide an example of the probe.

%1.SUBMISSION TO THE MANAGED CLOUD
The developer does not only develop the microservice itself but also the probes, which both are required for the submission of the microservice to the managed edge cloud environment. The probe is an inputless function that is used to measure the performance of a subset of operations of the microservice that needs to be guaranteed. It provides a means of balancing the need for prior knowledge and black-boxiness of the application. The microservice timing requirements and edge-cloud guarantees are expressed over those probes. Which means that the edge-cloud guarantees relate to the probes and not the microservice itself.

%The probe performance is measured in the edge-cloud. 

%they provide a way how to avoid slowing down the real application by taking measurements during its runtime.
 

In Listing \ref{lst:deployment-descriptor}, which represents the deployment descriptor, we can see the mandatory timing requirement definition for two probes: RecognizePeople and DetectHeads.

During the submission process of the microservice to the edge-cloud probes have an essential role. In comparison to a typical cloud environment submission, our solution has an extra step of approval phase. In this step, probes are measured, and results are evaluated against probes timing requirements to determine whether the edge-cloud could provide the required guarantees. The developer is informed on the outcome (i.e., admission successful with such and such price, or unsuccessful because the requirements can't be fulfilled) only after this step is the process of submission completed. 

%*alternatively (when the time requirements do not have to be specified) the assessment in the cloud could also provide offers of guarantees in different price and latency levels tailored for the specific microservice. (e.g., for our application the response time in a setup: 90\% of requests would have a response within 90ms and 99\% within 180ms would cost 5\$ or 90\% of requests would have a response within 30ms and 99\% within 90ms would cost 25\$ ).

%2.HOW SHOULD THE PROBE LOOK LIKE
%We can think about it as an usecase scenario that uses most of the important features or the most expensive one
The probe itself is a mockup procedure that should cover the essential parts of the application behavior. The complete set of probes should reach all possible use case scenarios to cover all resource expensive parts of the service. The probe would not function as microservice which waits for user input that is then processed. Instead, the function should include pre-defined user input so it could be without any parameters and would be executed immediately upon the call.
In the probe context, we are not interested in network latency. Although the application itself may try to minimize it, e.g., video application could decrease the image resolution, but such case should be part of another probe. Since the network is, as seen of our perspective, almost 
unlimited % maybe explain why???
medium, the input may be hard-coded within the probe or taken from a hard drive. The output of the probe is not used so it could be omitted altogether. 
It should not change the outer application state so that the there would be consistency in between the runs of the probes.
%* initialization stage, cleaning stage -- before and after the run???
If a database is part of the functioning of the probe, then it is needed the include a staging database. To achieve close-to-real database performance measurements, it is advisable for the database to be of a reasonably large size.

%3.EXAMPLE OF THE PROBE
A probe for our motivation example with the timing requirements from RecognizePeople would consist of the identification of faces in the image and lookup of names in a database. A set of images will be part of the probe itself so that no input would be required. The recognition will be done over randomly selected image from the set, and the lookup would be performed in a staging database which would also be part of the probe. A probe for DetectHeads would be similar but would lack the database parts. Purpose of this functionality is to achieve same result as the function known from the cameras, which draws the rectangle around the head, here the result would be a set of squares coordinates for each head in the image.


